A Limitation of the PAC-Bayes Framework

PAC-Bayes is a useful framework for deriving generalization bounds which was introduced by McAllester ('98). This framework has the flexibility of deriving distribution- and algorithm-dependent bounds, which are often tighter than VC-related uniform convergence bounds. In this manuscript we present a limitation for the PAC-Bayes framework. We demonstrate an easy learning task that is not amenable to a PAC-Bayes analysis. Specifically, we consider the task of linear classification in 1D; it is well-known that this task is learnable using just $O(\log(1/\delta)/\epsilon)$ examples. On the other hand, we show that this fact can not be proved using a PAC-Bayes analysis: for any algorithm that learns 1-dimensional linear classifiers there exists a (realizable) distribution for which the PAC-Bayes bound is arbitrarily large.

==> drafts.tex <==

Let $\D$ be a random uniform distribution over the domain $\X_{k}$ and $y=1$ iff $x$ is smaller than $k/2$. We will show that this candidate distribution yields \cref{thm:main}.

We begin the proof by depicting the process of randomly choosing a well -ordered sample in a slightly different manner. Specifically, consider the distribution $\U$ supported on triplets $(j,\order{S},\hat{x})$ where $j\in [m]$, $\order{S}$ is an ordered sample and $\hat{x}\in [x_{i-1},x_{i+1}]$:
\begin{enumerate}
\item\label{it:1} First we pick the threshold sign pattern $j$ and an order $\pi$ according to $\D^{m}$ (in other words, $j$ is chosen with probability $p$ if the probability to draw an i.i.d sample with threshold sign-pattern $j$ and order $\pi$ is $p$).
\item\label{it:2} We then pick an ordered sample $\order{S}$ according to $\D^m(\cdot |j)$, (i.e. we pick a sample $S$ according to $\D^m$ conditioned on the sign pattern, and we order it to obtain $\order{S}$).
\item\label{it:3} Then, if there exists $i$ such that $|p^{(\pi,j)}_{i-1}-p^{\pi,j}_{i,j}|\ge \gamma /(2m)$, we pick an element $\hat{x}$, chosen uniformly from the interval\footnote{if more then one $i$ satisfies the above condition, we pick the first} $[x_{i-1},x_{i+1}]$ but without changing the sign pattern. 
More formally, we pick uniformly at random from the interval $I(\order{S})$ where

\begin{align}\label{eq:interval} I(\order{S})= \begin{cases}
[x_{i-1},x_{i+1}] & k/2\notin [x_{i-1},x_{i+1}]\\
[x_{i-1},k/2] & (x_{i-1}\le x_i\le k/2\le x_{i+1})\\
[k/2, x_{i+1}] & (x_{i-1}\le k/2\le x_i\le x_{i+1})
\end{cases}.\end{align}
If no such $i$ exists we let $\hat{x}=x_i$.

\end{enumerate}
Let $\S_{\hat{x}}$ be sample obtained by picking $(j,\order{S},\hat{x},\pi)\sim \U$,  and then replacing $x_i$ with $\hat{x}$ and finally applying the permutation $\pi$ on the sample. Namely:
\begin{align}\label{eq:Spix} S^{\pi}_{\hat{x}}
=
\langle (x_{\pi(1)},y_{\pi(1)}),
(x_{\pi(2)},y_{\pi(2)}),\ldots, ,\underbrace{(\hat{x},y_i)}_{\textrm{$\pi^{-1}(i)$-coordinate}},\ldots, (x_{\pi(m)},y_{\pi(m)}\rangle.\end{align}

It is easy to see that the above process is equivalent to simply picking a sample $S$ from $\D^m$. Thus \cref{thm:main} will follow from the following claim:


\begin{claim}
Let $A$ be an homogeneous posterior-learning algorithm. Let $(j,\pi,\order{S},\hat{x})\sim \U$, where $\U$ is the distribution described by the random process depicted in \cref{it:1,it:2,it:3}. 

Also, let $S^{\pi}_{\hat{x}}$ be the sample obtained from $(\order{S},\pi,\hat{x})$ as depicted in \cref{eq:Spix}, then with probability $2/3$, we have that either

\end{claim}
